The E00-110 experiment in Jefferson Lab's Hall A: Deeply Virtual Compton Scattering off the Proton at 6 GeV

We present final results on the photon electroproduction ($\vec{e}p\rightarrow ep\gamma$) cross section in the deeply virtual Compton scattering (DVCS) regime and the valence quark region from Jefferson Lab experiment E00-110. Results from an analysis of a subset of these data were published before, but the analysis has been improved which is described here at length, together with details on the experimental setup. Furthermore, additional data have been analyzed resulting in photon electroproduction cross sections at new kinematic settings, for a total of 588 experimental bins. Results of the $Q^2$- and $x_B$-dependences of both the helicity-dependent and helicity-independent cross sections are discussed. The $Q^2$-dependence illustrates the dominance of the twist-2 handbag amplitude in the kinematics of the experiment, as previously noted. Thanks to the excellent accuracy of this high luminosity experiment, it becomes clear that the unpolarized cross section shows a significant deviation from the Bethe-Heitler process in our kinematics, compatible with a large contribution from the leading twist-2 DVCS$^2$ term to the photon electroproduction cross section. The necessity to include higher-twist corrections in order to fully reproduce the shape of the data is also discussed. The DVCS cross sections in this paper represent the final set of experimental results from E00-110, superseding the previous publication.

==> biblio.tex <==
\begin{thebibliography}{}

\bibitem{rad96} A.V.\ Radyushkin, 
%``Asymmetric gluon distributions and hard diffractive electroproduction,''
Phys.\ Lett.\ B {\bf 385}, 333 (1996)
[hep-ph/9605431]. %;

\bibitem{ji96} X.~-D.~Ji,
  %``Deeply virtual Compton scattering,''
  Phys.\ Rev.\ D {\bf 55}, 7114 (1997)
  [hep-ph/9609381].
  %%CITATION = HEP-PH/9609381;%%

\bibitem{col96} J.C.\ Collins, L.\ Frankfurt and M.\ Strikman, 
%``Factorization for hard exclusive electroproduction of mesons in QCD,''
Phys.\ Rev.\ D {\bf 56}, 2982 (1997)
[hep-ph/9611433].
%%CITATION = HEP-PH 9611433;%%

\bibitem{collins99} 
  J.~C.~Collins and A.~Freund,
  %``Proof of factorization for deeply virtual Compton scattering in QCD,''
  Phys.\ Rev.\ D {\bf 59}, 074009 (1999)
  [hep-ph/9801262].
  %%CITATION = HEP-PH/9801262;%%
 
\bibitem{muller94} D.~Mueller, D.~Robaschik, B.~Geyer, F.~M.~Dittes and 
J.~Horejsi,
  %``Wave functions, evolution equations and evolution kernels from light 
% ray operators of QCD,''
  Fortsch.\ Phys.\  {\bf 42}, 101 (1994)
  [hep-ph/9812448].
  %%CITATION = HEP-PH/9812448;%%

\bibitem{rad97} 
  A.~V.~Radyushkin,
  %``Nonforward parton distributions,''
  Phys.\ Rev.\ D {\bf 56}, 5524 (1997)
  [hep-ph/9704207].
  %%CITATION = HEP-PH/9704207;%%

\end{thebibliography}
